Integrals over Hilbert schemes and multiple $q$-zeta values

We establish a version of Okounkov's conjecture on multiple $q$-zeta values arising from integrals over Hilbert schemes of points on smooth projective surfaces. We prove that normalized generating series of integrals involving products of Chern characters of tautological bundles belong to the algebra $\mathcal Z_q$ of multiple $q$-zeta values, without restrictions on the canonical class of the surface. The proof combines vertex-operator methods with a reduction to graph sums, whose arithmetic structure is governed by the cohomology of the surface. We also derive a closed universal formula for the Chern character operators acting on the cohomology of Hilbert schemes by solving a system of differential equations arising from Lehn's commutator relations.

==> commands.tex <==
\RequirePackage{amsmath,amssymb,amsthm}
\RequirePackage{etoolbox,xspace,scalerel}
\RequirePackage{version,xparse}
\RequirePackage[capitalize]{cleveref}
\makeatletter

%%%% Theorem environments
%\ifx\theorem\undefined
\ifundef\theorem{
  \newtheorem{thm}{Theorem}[section]
  \def\newthmx#1#2{
    \ifcsundef{#1}{
      \newtheorem{#1}[thm]{#2}
      \AddToHook{env/#1/begin}{\crefalias{thm}{#1}} %fix cleveref
    }{}
  }
  \def\newthm#1{\newthmx{#1}{\MakeUppercase#1}}

  \theoremstyle{plain}
  \forcsvlist\newthm{theorem,lemma,corollary,proposition,conjecture}
  \theoremstyle{definition}
  \forcsvlist\newthm{definition,remark,example,question,claim,exercise}
  \theoremstyle{remark}
  \newthmx{rmr}{Remark}
}{}

% References
\numberwithin{equation}{section} %before thmtools, hyperref?

%%%% Auxiliary commands
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}} %define math command
\def\csdmat#1#2{\csdef{#1}{\mat{#2}}}
\def\opn{\operatorname}
\def\opr#1#2{\dmat#1{\opn{#2}}}
\def\DMO{\opr}
\def\csopr#1#2{\csdmat{#1}{\opn{#2}}}
\def\oper#1{\csopr{#1}{#1}}
\def\operl{\forcsvlist\oper}
\def\redef#1{\csletcs{t@#1}{#1}\csdmat{#1}{\csuse{t@#1}}}
\newcommand\envalias[2]{\newenvironment{#1}{\begin{#2}}{\end{#2}}}


%%%% Operators. Usage: \GL
\forcsvlist\oper{
Vect,Mod,Rep,Ab,Grp,Com,Set,Top,Sch,Coh,Qcoh,Ob,Ring,Alg,
Map,Hom,End,Aut,Ext,Cat,Sh,Ind,RHom,Fun,Var,rad,
Ker,Im,Re,deg,Tr,det,rk,diag,im,coker,tr,cone,add,
sk,cosk,colim,Res,Gal,Coker,dlog,sgn,Li,
GL,SL,PGL,Gr,Lib,Conv,Sol,Tor,
Max,Spec,Proj,Ass,Ann,Quot,Pic,Sym,MHS,MHM,
td,Td,ch,Supp,supp,vol,trdeg,lc,NS,Loc,Iso,per,gr,Der,Lie,
Log,Exp,Pow,ord,lcm,VB,Hilb,cl,SU,SO,Ad,ad,id,Span,Arg,Bl,wt,Cone,
coim,Coim,eq,coeq,Eq,Coeq}

\opr\Id{id}
\opr\lHom{\lb{Hom}}
\opr\lEnd{\lb{End}}
\opr\lAut{\lb{Aut}}
\opr\lIso{\lb{Isom}}
\opr\hgt{ht}
\opr\chr{char}
\opr\udim{\mathbf{dim}}
\opr\cls{\mathsf{cl}}
\opr\mmod{mod}
\opr\Et{\mathsf{Et}}
\def\sign{\sgn}
\opr\spn{span}

\dmat\Gm{\mathbb G_{\mathrm m}}
\dmat\pt{\mathbf{pt}}
\def\opfrak#1{\csdef{#1}{\mathfrak{#1}}}
\forcsvlist\opfrak{gl,sl,su,so}
\def\oprm#1{\csdef{#1}{\mathrm{#1}}}
\forcsvlist\oprm{op,nil,et,sep,ab,top,tf,}
\def\st{\mathrm{s}}
\def\sst{\mathrm{ss}}
\def\Ta{T^{\mathrm a}} %tensor algebra
\def\Tc{T^{\mathrm c}} %tensor coalgebra
\def\Vecf{\Vect_{\mathrm f}}

%%%% Arrows
\def\mto{\mapsto}
\def\xto{\xrightarrow}
\def\lto{\leftarrow}
\def\emb{\hookrightarrow}
\def\lemb{\hookleftarrow}
\def\onto{\twoheadrightarrow}
\RequirePackage{mathtools}
\def\xmto{\xmapsto}
\def\xlto{\xleftarrow}
\def\xemb{\xhookrightarrow}
\def\xonto#1{\xto{#1}\mathrel{\mkern-14mu}\to}
\def\dashto{\dashrightarrow}
\def\dto{\dashrightarrow}
\def\dashlto{\dashlefttarrow}
\def\dlto{\dashlefttarrow}

%%% Symbols
\redef{iff}
\dmat\imp{\implies}
\dmat\es{\varnothing}%{\emptyset}
\def\bs{\backslash}
\def\ms{\backslash}
\def\sbs{\subset}
\def\sps{\supset}
\def\sbe{\subseteq}
\def\spe{\supseteq}
\dmat\xx{\times}
\dmat\Cx{\bC^\times}
\dmat\dd{\partial}
\def\pd#1{\frac\dd{\dd#1}}
\def\iso{\simeq}
\def\isoc{\cong} %canonical isomorphism
%\def\bop{\bigoplus}
\def\ilim{\varprojlim} %inverse limit
\def\dlim{\varinjlim} %direct limit
\def\ts{\otimes}
%\def\bts{\bigotimes}
\def\lb{\underline}
\def\ub{\overline}
\NewDocumentCommand\ubar{O{1.5}O{1.5}m}{%
  \mkern#1mu\overline{\mkern-#1mu#3\mkern-#2mu}\mkern#2mu}

\def\oh{{\frac12}}
\def\toh{{\tfrac12}}
\RequirePackage{bbm}
\dmat\one{\mathbbm1} %requires bbm
\def\qt{\delimiter"502F30E\mathopen{}} %/correct spacing
\def\partof{\vdash}
\def\adj{\mathrel{\tikz
\draw[line cap=round](0,0)--(0,1.5ex)(0,.75ex)--(-1.5ex,.75ex);}}
%\def\adj{\mathrel{\relbar\mkern-14mu\vcenter{\hbox{$\dashv$}}}}
\def\what{\widehat}
\def\tl{\tilde}
\def\wtl{\widetilde}
\def\inv{^{-1}}
\def\trp{^{\mathsf T}} %transpose
\dmat\bul{\bullet}
\def\GIT{/\!\!/}
\def\git{\GIT}
\def\qbinom{\genfrac{[}{]}{0pt}{}}
\def\m{\wedge}
\def\j{\vee}
\def\blank{\scalebox{.8}{$-$}} %blank argument

\def\upc{\tikz{\draw[->,>=latex'](0,0)--(0,.3)}}
%requires \usetikzlibrary{arrows}
\def\upc#1{\left\uparrow#1\right.}%upper closure
\def\loc#1{\left\downarrow#1\right.}%lower closure
\def\cupp{\!\smallsmile\!} %cup product
\def\capp{\!\smallfrown\!} %cap product

\def\vcenterx#1{\vcenter{\hbox{#1}}}
\def\rsbox#1#2#3{% raise and scale
  \raisebox{#1}{\scalebox{#2}{\ensuremath{#3}}}}
\NewDocumentCommand\cscale{O{0pt} O{.7} m}{%
  %Central scale: #1-raise, #2-scale, #3-argument
  \ThisStyle{\vcenterx{\rsbox{#1}{#2}{\SavedStyle#3}}}}


\def\isoto{\xto{\,\smash{\rsbox{-3pt}{.8}\sim}\,}}
%\def\dual{^{\cscale[.8]{\vee}}}
\def\dual{^{\scalerel*\vee{*}}}
\def\sbul{\cscale[1pt][.7]{\bullet}}
%\def\ac{{\tiny\raisebox{2pt}{\textup{!}}}}%anti-shriek?
\def\ac{{\scalerel*{\rotatebox[origin=c]{180}{!}}{!}}}

\usepackage[T2A]{fontenc} %T2A, OT2
%\def\sha{\mathord{\textup\cyrsh}}
\DeclareSymbolFont{cyrletters}{T2A}{cmr}{m}{n}
\DeclareMathSymbol{\sha}{\mathbin}{cyrletters}{\cyrsh}

\let\t@sum\sum
\def\sum{\@ifstar{\t@sum\nolimits}\t@sum}
\let\t@prod\prod
\def\prod{\@ifstar{\t@prod\nolimits}\t@prod}
\let\t@bop\bigoplus
\def\bop{\@ifstar{\t@bop\nolimits}\t@bop}
\def\bts{\@ifstar{\bigotimes\nolimits}\bigotimes}

\newcommand\tcd[2][]{%
  \begin{tikzcd}[#1,ampersand replacement=\&]#2\end{tikzcd}}

\newenvironment{ctikzcd}
	{\center\tikzcd}{\endtikzcd\endcenter}

\newcommand\edge[2][1.5em]{%\xrightarrow without tip
  \tcd[cramped,column sep=#1]{\rar[-,"#2"]\&{}}}


%%%% Aphabets: \bA,\cA,\fA,\bfA,\sA
\def\flist#1#2{\expandafter\forcsvlist\expandafter#1\expandafter{#2}}
\def\defbb#1{\csdmat{b#1}{\mathbb{#1}}}
\def\defcal#1{\csdmat{c#1}{\mathcal{#1}}}
\def\deffrak#1{\csdmat{f#1}{\mathfrak{#1}}}
\def\defbf#1{\csdmat{bf#1}{\mathbf{#1}}}
\def\defsf#1{\csdmat{s#1}{\mathsf{#1}}}
\def\defrm#1{\csdmat{r#1}{\mathrm{#1}}}
\def\defall#1{\defbb{#1}\defcal{#1}\deffrak{#1}\defbf{#1}%
  \defsf{#1}\defrm{#1}}

\forcsvlist\defall{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}
\forcsvlist\deffrak{a,b,c,d,e,f,g,h,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}

\def\deflbf#1{\csdmat{b#1}{\mathbf{#1}}} %lower case bf
\forcsvlist\deflbf{a,b,c,d,e,g,h,i,j,k,l,n,o,p,q,r,s,t,u,v,w,x,y,z}
\forcsvlist\defbf{f,k,m} %\bff,\bfk,\bfm
%\dmat\bk{\mathbbm k}
\dmat\bk{\Bbbk}
\defrm{i} %\ri


%%%% Greek letters
\dmat\al\alpha
\dmat\be\beta
\dmat\ga\gamma
\dmat\de\delta
\dmat\la\lambda
\dmat\ta\tau
\dmat\hi\chi
\dmat\eps\varepsilon
\dmat\ep\epsilon
\dmat\io{\iota}
\dmat\vi\phi
\dmat\te\theta
\dmat\ksi\xi
\dmat\si\sigma
\dmat\om\omega
\dmat\Ga\Gamma
\dmat\La\Lambda
\dmat\De\Delta
\dmat\Om\Omega
\dmat\Si{\Sigma}
\dmat\ze\zeta
\dmat\Te{\Theta}
\dmat\Na{\nabla}
\dmat\kp{\kappa}
\forcsvlist\redef{Phi,Psi,pi,mu,nu,rho}

%%%% Structures
\RequirePackage{mleftright} %better spaces
\def\lr#1#2#3{\mleft#1#2\mright#3}
\def\set#1{\lr\{{#1}\}}
%\def\sets#1#2{\set{#1\,\lr|{\,\vphantom{#1}#2}.}}
\def\sets#1#2{\set{#1\,\middle|\,#2}}
\def\setc#1#2{\set{#1\col#2}}
\def\ang#1{\lr\langle{#1}\rangle}
\def\angs#1#2{\ang{#1\col#2}}
\def\rbr#1{\lr({#1})} %round bracket
\def\sbr#1{\lr[{#1}]} %square bracket
\def\brc{\set} %curly bracket, braces
\def\cbr{\set}
\def\emp{\cdot,\cdot} %empty parameters
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\n#1{\left\lvert#1\right\rvert}
\def\nn#1{\left\lVert#1\right\rVert}

\def\rbig#1{\big(#1\big)}
\def\rBig#1{\Big(#1\Big)}
\def\rbigg#1{\bigg(#1\bigg)}
\def\rBigg#1{\Bigg(#1\Bigg)}
\def\sth#1#2{\lr.{#1}|_{#2}}
\def\sbig#1{\big[#1\big]}
\def\sBig#1{\Big[#1\Big]}
\def\sbigg#1{\bigg[#1\bigg]}


\def\nspc#1{\hspace{-2.5pt}#1\hspace{-2.5pt}}%neg. space
\def\pser#1{[\![#1]\!]} %formal power series [[#1]]
\def\lser#1{(\nspc{(#1)})} %formal Laurent series ((#1))
\def\cps#1{\{#1\}} %convergent power series
\def\cls#1{(\nspc{\cps{#1}})} %convergent Laurent series
\def\angg#1{\ang{\nspc{\ang{#1}}}}
%\def\nop#1{\left.\col\nspc{#1}\col\right.}%normally ordered product
%\def\nop#1{\,{\col#1\,\col}\,}   %% normally ordered
\def\scol#1{\scalebox{#1}{\ensuremath\col}} %scale column
\def\scalemacro#1{\mathchoice{#1{1.2}}{#1{1.2}}{#1{1}}{#1{1}}}
\def\nop#1{\,\scalemacro\scol#1\scalemacro\scol\,}


\def\matr#1{\begin{matrix}#1\end{matrix}}
\def\pmat#1{\begin{pmatrix}#1\end{pmatrix}}
\def\bmat#1{\begin{bmatrix}#1\end{bmatrix}}
\def\vmat#1{\begin{vmatrix}#1\end{vmatrix}}
\def\smatr#1{\begin{smallmatrix}#1\end{smallmatrix}}
\def\smat#1{\rbr{\smatr{#1}}}
\def\pmatv#1#2{\left(\matr{#1}
	\hspace{.5ex}\middle|\hspace{.3ex}
	\matr{#2}\right)}
\def\ov#1#2{{\substack{#1\\#2}}} % #1 over #2
%\def\eq#1{\begin{equation}#1\end{equation}} %used for equalizers
\RequirePackage{mathtools}
\def\ctr{\overbracket[.5pt][2pt]} %contraction, requires mathtools


%%%% Diff
\def\brake{\ \vspace{-.5ex}} %break after itemize
\def\dir#1#2{\noindent\textbf{(#1)$\imp$(#2).}}
\def\ddir#1#2{\noindent\textbf{(#1)$\iff$(#2).}}
\def\clm#1{\noindent\textbf{(#1)}\xspace} %claim, \cl should be used for classes
\def\lqq{\lq\lq}
\def\rqq{\rq\rq\xspace}
\def\qq#1{\lqq#1\rqq}
\def\tpdf{\texorpdfstring} %hyperref
\def\hl{\noindent\rule{\textwidth}{1pt}}

%%%% Words and phrases
%\def\ie{i.e.,\,} %id est
%\def\eg{e.g.\@\xspace} %exempli gratia
%\def\cf{cf.\@\xspace} %confer
\def\ie{i.e.\@\xspace} %id est
\def\eg{e.g.\ } %exempli gratia
\def\cf{cf.\ } %confer
\def\lci{l.c.i.\@\xspace}
\def\etale{\'etale\xspace}
\def\qis{quism\xspace} %quasi-isomorphism
\def\wrt{with respect to\xspace}
\def\hint{\noindent\textbf{Hint:}\xspace}
%\def\wlog{without loss of generality\xspace}
\def\Wlog{Without loss of generality\xspace}
\def\fae{following are equivalent\xspace}
\def\tfae{the \fae}
\def\nbd{neighborhood\xspace}
\def\fdd{finite-dimensional\xspace} % \fd used for \mathfrak{d}
\def\ifft{if and only if\xspace}

%%%% Citations
\def\defcite#1#2{%\defcite\moz{mozgovoy_DT}
	\DeclareDocumentCommand{#1}{o}
		{\IfValueTF{##1}{\cite[##1]{#2}}{\cite{#2}}\xspace}
}
\def\eprint#1{\href{https://arxiv.org/abs/#1}{\ttfamily#1}}

%%%% Colons
\mathchardef\col=\mathcode`:
\mathchardef\eqsymb=\mathcode`=
\def\ordinarycolon{\col} %used in \coloneqq and \vcentcolon
\AtBeginDocument{\mathcode`:="8000\mathcode`=="8000}
\RequirePackage{mathtools} %for \coloneqq

\def\colona{\nobreak\mskip2mu\mathpunct{}%\nonscript
  \mkern-\thinmuskip{\col}
  \mathchoice{\mskip6mu plus1mu}{\mskip6mu plus1mu}{\mskip1mu}{}
}
\def\colon{\colona}

\makeatletter
\def\activecolon{\@ifnextchar={\coloneqq\@gobble}{\colona}}
\def\activeequal{\@ifnextchar:{\eqqcolon\@gobble}{\eqsymb}}
\makeatother
{ \catcode`:=\active\gdef:{\activecolon}
  \catcode`==\active\gdef={\activeequal}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Indexed definition \idef{name}{optional name}
\DeclareDocumentCommand{\idef}{mo}{%
  \ifstrempty{#1}{}{\ifmmode#1\else\emph{#1}\fi}%
	\IfValueTF{#2}{\index{#2}}{\index{#1}}%
}

%%% Notes
\ifx\note\undefined
\RequirePackage[framemethod=TikZ]{mdframed}
\mdfsetup{backgroundcolor=brown!10, linewidth=0,
  skipabove=5pt, roundcorner=5pt}

\theoremstyle{definition}
\newmdtheoremenv[innertopmargin=-2pt]{note}{Note}
\newenvironment{notes}{\begin{note}}{\end{note}}

\newenvironment{comm}[1][brown!10]
  {\begin{mdframed}[backgroundcolor=#1]}{\end{mdframed}}
\newcommand\memo[2][brown!10]{
  \begin{mdframed}[backgroundcolor=#1]#2\end{mdframed}}
\def\red#1{\textcolor{red}{#1}}
\fi

%custom number side in equations, manual number: \tag{name}
\makeatletter
\def\leqnomode{\tagsleft@true\let\veqno\@@leqno}
\def\reqnomode{\tagsleft@false\let\veqno\@@eqno}
\makeatother


%custom theorem, can be used to list axioms (with labels)
\ifx\customthm\undefined
\theoremstyle{plain}
\newtheorem{innercustomthm}{}
\newenvironment{customthm}[1]
  {\def\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
\fi

% short names for theorems
\def\shortThm{
\envalias{thm}{theorem}
\envalias{thr}{theorem}
\envalias{dfn}{definition}
\envalias{lmm}{lemma}
\envalias{crl}{corollary}
\envalias{prp}{proposition}
}

\makeatother

%%%% Tikz %%%%
%\long\def\command#1{\providecommand{#1}{}\renewcommand{#1}}
\def\vcenterx#1{\ensuremath{\vcenter{\hbox{#1}}}}
\newcommand\btikz[2][]{\vcenterx{\tikz[#1]{#2}}} %base line
\newcommand\ctikz[2][]{\begin{center}\tikz[#1]{#2}\end{center}}

\def\eq#1{\begin{equation}#1\end{equation}}
\def\i{^{-1}}

%%% Redefine \newcommand
%\makeatletter
%\let\oldcomm\newcommand
%\def\newcommand{\@ifstar{\oldcomm}{\newcomm}}
%\def\newcomm#1{
%  \@ifundefined{\expandafter\@gobble\string#1}
%    {\oldcomm{#1}}{\renewcommand{#1}}%
%}


